Neural networks can understand compositional functions that humans do not, in the context of emergent communication

We show that it is possible to craft transformations that, applied to compositional grammars, result in grammars that neural networks can learn easily, but humans do not. This could explain the disconnect between current metrics of compositionality, that are arguably human-centric, and the ability of neural networks to generalize to unseen examples. We propose to use the transformations as a benchmark, ICY, which could be used to measure aspects of the compositional inductive bias of networks, and to search for networks with similar compositional inductive biases to humans. As an example of this approach, we propose a hierarchical model, HU-RNN, which shows an inductive bias towards position-independent, word-like groups of tokens.

==> 4_related_work.tex <==
% \section{Related work}

% Examples of emergent communication were presented in \ref{section:introduction}. Existing work on metrics for measuring compositionality was presented in \ref{section:compositionality}.

% Our work relates also to probe models such as \citet{hewitt2019structural} and \citet{tenney2019you}, which probe for compositional structure in the contextualized word representations output from pre-trained BERT models \citep{devlin2018bert}. By contrast, we examine the ease with which a model can learn pre-defined compositional grammars. Our work relates also to \citet{tenney2019bert} which probes the extent to which latent language features can be detected at each layer of a pre-trained BERT model.

% Examples of emergent communication were presented in our `Introduction' section, whilst existing work on metrics for measuring compositionality was presented in our `Background' section.


==> figures/learning_architectures.tex <==
% \begin{table}[htb!]
% \small
% \centering
%     \begin{tabular}{@{}p{0.14\linewidth}p{0.78\linewidth}@{}}
%     \toprule
%         Name & Description \\
%         \midrule
%         % RNNZero:* & Sender RNN with zero'd inputs \\
%         % RNNAutoReg:* & Autoregressive sender RNN \\
%         % RNNSampling:* & Sender RNN with sampling \\
%         % RNN:* & Receiver RNN \\
%         % HU:* & Hierarchical receiver \\
%         % HUZero:* & Hierarchical sender with zero'd inputs \\
%         % HUAutoReg:* & Autoregressive hierarchical sender \\
%         % *:RNN & Vanilla RNN Cell \\
%         % *:GRU & GRU RNN Cell \\
%         % *:SRU & SRU RNN Cell \citep{sru} \\
%         FC & Fully connected network \\
%         LSTM & LSTM RNN \\
%         dgsend & Sender RNN evolved in \citet{dagan2020co} \\
%         *1L & postfix denoting 1 layer \\
%         *2L & postfix denoting 2 layers \\
%         % FC1L & 1 Layer fully connected network \\
%         % FC3 & 3 layer fully connected \\
%         % *:dgrecv & Receiver cell evolved from \citet{dagan2020co} \\
%         CNN & convolutional network \\
%         TransDec & Transformer decoder \\
%         hash & hashtable \\
%         % kNN & k nearest neighbors \\
%     \bottomrule
%     \end{tabular}
%     \caption{Learning architectures under test.}
%     \label{tab:learning_architectures} 
% \end{table}


==> tables/sender_3x10.tex <==
% \begin{table}
% \begin{tabular}{lllllll}
% \toprule
% Neural model & Params & \textsc{proj} & \textsc{perm} & \textsc{rot} & \textsc{shufdet} & \textsc{hol} \\
% \midrule
% FC1L & 1860 & 2.6 & 0.9 & > 20 & 2.3 & > 20 \\
% FC2L & 11708 & 3 & 1 & > 20 & 2.5 & > 20 \\
% LSTM1L & 137349 & 1.6 & 1 & 1.9 & 1.2 & 6.5 \\
% LSTM2L & 269445 & 1.8 & 1.3 & 2.3 & 1.6 & 4.6 \\
% dgsend & 103557 & 1.4 & 1 & 1.9 & 1 & 4.4 \\
% TransDecSoft1L & 269829 & 2.6 & 1.2 & 3.1 & 1.7 & > 20 \\
% TransDecSoft2L & 534405 & 2.2 & 0.9 & 3.3 & 1.3 & 9.5 \\
% Hashtable & O(N) & 1 & 1 & 1 & 1 & 1 \\
% \bottomrule
% \end{tabular}
% \caption{Acquisition time relative to \textsc{comp}, i.e. $b = \frac{N_{acquire}^{\mathcal{G}} } { N_{acquire}^{\mathcal{\textsc{comp}}} }$}
% \label{fig:sender_3x10}
% \end{table}

% \begin{table}
% \begin{tabular}{lp{0.24\linewidth}llllll}
% \toprule
% Model & Description & Params & \textsc{proj} & \textsc{perm} & \textsc{rot} & \textsc{shufdet} & \textsc{hol} \\
% \midrule
% FC1L & 1-layer fully-connected & 1860 & 2.6 & 0.9 & > 20 & 2.3 & > 20 \\
% FC2L & 2-layer fully-connected & 11708 & 3 & 1 & > 20 & 2.5 & > 20 \\
% LSTM1L & 1-layer LSTM & 137349 & 1.6 & 1 & 1.9 & 1.2 & 6.5 \\
% LSTM2L & 2-layer LSTM & 269445 & 1.8 & 1.3 & 2.3 & 1.6 & 4.6 \\
% dgsend & Sender RNN evolved in \citet{dagan2020co} & 103557 & 1.4 & 1 & 1.9 & 1 & 4.4 \\
% Trans1L & Transformer decoder 1-layer & 269829 & 2.6 & 1.2 & 3.1 & 1.7 & > 20 \\
% Trans2L & Transformer decoder 2-layer & 534405 & 2.2 & 0.9 & 3.3 & 1.3 & 9.5 \\
% Hashtable & Hashtable & O(N) & 1 & 1 & 1 & 1 & 1 \\
% \bottomrule
% \end{tabular}
% \caption{Acquisition time relative to \textsc{comp}, i.e. $b = \frac{N_{acquire}^{\mathcal{G}} } { N_{acquire}^{\mathcal{\textsc{comp}}} }$}
% \label{fig:sender_3x10}
% \end{table}

\begin{table}
\small
\caption{Acquisition time relative to \textsc{comp}, i.e. $b = \frac{N_{acquire}^{\mathcal{G}} } { N_{acquire}^{\mathcal{\textsc{comp}}} }$, for candidate Sender models}
\begin{tabular}{p{0.37\linewidth}llllll}
\toprule
Model & Params & \textsc{perm} & \textsc{proj} & \textsc{rot} & \textsc{shufdet} & \textsc{hol} \\
\midrule
1-layer MLP \citep{rumelhart1986learning} & 1860 & \textcolor{green!50!black!50}{0.9} & \textcolor{green!50!black!50}{2.6} & \textcolor{red}{> 20} & \textcolor{green!50!black!50}{2.3} & \textcolor{red}{> 20} \\
2-layer MLP & 11708 & \textcolor{green!50!black!50}{1} & \textcolor{green!50!black!50}{3} & \textcolor{red}{> 20} & \textcolor{green!50!black!50}{2.5} & \textcolor{red}{> 20} \\
1-layer LSTM \citep{hochreiter1997long} & 137349 & \textcolor{green!50!black!50}{1} & \textcolor{green!50!black!50}{1.6} & \textcolor{green!50!black!50}{1.9} & \textcolor{green!50!black!50}{1.2} & 6.5 \\
2-layer LSTM & 269445 & \textcolor{green!50!black!50}{1.3} & 1.8 & 2.3 & 1.6 & 4.6 \\
Sender RNN evolved in \citet{dagan2020co} & 103557 & \textcolor{green!50!black!50}{1} & \textcolor{green!50!black!50}{1.4} & 1.9 & \textcolor{green!50!black!50}{1} & 4.4 \\
1-layer Transformer decoder \citep{vaswani2017attention} & 269829 & \textcolor{green!50!black!50}{1.2} & \textcolor{green!50!black!50}{2.6} & \textcolor{green!50!black!50}{3.1} & \textcolor{green!50!black!50}{1.7} & \textcolor{red}{> 20} \\
2-layer Transformer decoder & 534405 & \textcolor{green!50!black!50}{0.9} & \textcolor{green!50!black!50}{2.2} & 3.3 & \textcolor{green!50!black!50}{1.3} & 9.5 \\
Hashtable & O(N) & 1 & 1 & 1 & 1 & 1 \\\bottomrule
\end{tabular}
\label{tab:sender_3x10}
\end{table}

% \begin{table}
% \begin{tabular}{lp{0.2\linewidth}lllllll}
% \toprule
% Model & Description & Layers & Params & \textsc{proj} & \textsc{perm} & \textsc{rot} & \textsc{shufdet} & \textsc{hol} \\
% \midrule
% FC1L & fully-connected & 1 & 1860 & 2.6 & 0.9 & > 20 & 2.3 & > 20 \\
% FC2L & ully-connected & 2 & 11708 & 3 & 1 & > 20 & 2.5 & > 20 \\
% LSTM1L & LSTM &1  & 137349 & 1.6 & 1 & 1.9 & 1.2 & 6.5 \\
% LSTM2L & LSTM & 2 & 269445 & 1.8 & 1.3 & 2.3 & 1.6 & 4.6 \\
% dgsend & Sender RNN evolved in \citet{dagan2020co} & 1 & 103557 & 1.4 & 1 & 1.9 & 1 & 4.4 \\
% Trans1L & Transformer decoder & 1 & 269829 & 2.6 & 1.2 & 3.1 & 1.7 & > 20 \\
% Trans2L & Transformer decoder & 2 & 534405 & 2.2 & 0.9 & 3.3 & 1.3 & 9.5 \\
% Hashtable & Hashtable & & O(N) & 1 & 1 & 1 & 1 & 1 \\
% \bottomrule
% \end{tabular}
% \caption{Acquisition time relative to \textsc{comp}, i.e. $b = \frac{N_{acquire}^{\mathcal{G}} } { N_{acquire}^{\mathcal{\textsc{comp}}} }$}
% \label{fig:sender_3x10}
% \end{table}

% \begin{table}
% \begin{subtable}{0.3\linewidth}
%     \begin{tabular}{@{}p{0.16\linewidth}p{0.8\linewidth}@{}}
%     \toprule
%         Name & Description \\
%         \midrule
%         % RNNZero:* & Sender RNN with zero'd inputs \\
%         % RNNAutoReg:* & Autoregressive sender RNN \\
%         % RNNSampling:* & Sender RNN with sampling \\
%         % RNN:* & Receiver RNN \\
%         % HU:* & Hierarchical receiver \\
%         % HUZero:* & Hierarchical sender with zero'd inputs \\
%         % HUAutoReg:* & Autoregressive hierarchical sender \\
%         % *:RNN & Vanilla RNN Cell \\
%         % *:GRU & GRU RNN Cell \\
%         % *:SRU & SRU RNN Cell \citep{sru} \\
%         FC & Fully connected network \\
%         LSTM & LSTM RNN \\
%         dgsend & Sender RNN evolved in \citet{dagan2020co} \\
%         *1L & postfix denoting 1 layer \\
%         *2L & postfix denoting 2 layers \\
%         % FC1L & 1 Layer fully connected network \\
%         % FC3 & 3 layer fully connected \\
%         % *:dgrecv & Receiver cell evolved from \citet{dagan2020co} \\
%         CNN & convolutional network \\
%         Trans & Transformer decoder \\
%         hash & hashtable \\
%         % kNN & k nearest neighbors \\
%     \bottomrule
%     \end{tabular}
% \end{subtable}
% \begin{subtable}{0.45\linewidth}
% \begin{tabular}{lllllll}
% \toprule
% Neural model & Params & \textsc{proj} & \textsc{perm} & \textsc{rot} & \textsc{shufdet} & \textsc{hol} \\
% \midrule
% FC1L & 1860 & 2.6 & 0.9 & > 20 & 2.3 & > 20 \\
% FC2L & 11708 & 3 & 1 & > 20 & 2.5 & > 20 \\
% LSTM1L & 137349 & 1.6 & 1 & 1.9 & 1.2 & 6.5 \\
% LSTM2L & 269445 & 1.8 & 1.3 & 2.3 & 1.6 & 4.6 \\
% dgsend & 103557 & 1.4 & 1 & 1.9 & 1 & 4.4 \\
% Trans1L & 269829 & 2.6 & 1.2 & 3.1 & 1.7 & > 20 \\
% Trans2L & 534405 & 2.2 & 0.9 & 3.3 & 1.3 & 9.5 \\
% Hashtable & O(N) & 1 & 1 & 1 & 1 & 1 \\
% \bottomrule
% \end{tabular}
% \end{subtable}
% \caption{Acquisition time relative to \textsc{comp}, i.e. $b = \frac{N_{acquire}^{\mathcal{G}} } { N_{acquire}^{\mathcal{\textsc{comp}}} }$}
% \label{fig:sender_3x10}
% \end{table}

